Clausal Resolution for Modal Logics of Confluence

We present a clausal resolution-based method for normal multimodal logics of confluence, whose Kripke semantics are based on frames characterised by appropriate instances of the Church-Rosser property. Here we restrict attention to eight families of such logics. We show how the inference rules related to the normal logics of confluence can be systematically obtained from the parametrised axioms that characterise such systems. We discuss soundness, completeness, and termination of the method. In particular, completeness can be modularly proved by showing that the conclusions of each newly added inference rule ensures that the corresponding conditions on frames hold. Some examples are given in order to illustrate the use of the method.

==> tables/table-axioms.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|}\hline
$(p,q,r,s)$ & Axiom & Usual Name \\ \hline
$(0,0,0,0)$ & $\varphi \then \varphi$ &  classical \\ \hline %--
$(0,0,0,1)$ & $\varphi \then \pos{\agent}\varphi$ &  \axiomname{T} \\ \hline %ok%ok
$(0,0,1,0)$ & $\varphi \then \nec{\agent}\varphi$ &  \axiomname{Ban} \\ \hline %ok%ok
$(0,0,1,1)$ & $\varphi \then \nec{\agent}\pos{\agent}\varphi$ &  \axiomname{B}\\ \hline %ok%ok
$(0,1,0,0)$ & $\nec{\agent}\varphi \then \varphi$ & \axiomname{T} \\ \hline % ok%ok
$(0,1,0,1)$ & $\nec{\agent}\varphi \then \pos{\agent}\varphi$ & \axiomname{D} \\ \hline % okok
$(0,1,1,0)$ & $\nec{\agent}\varphi \then \nec{\agent}\varphi$ & classical \\ \hline % --
$(0,1,1,1)$ & $\nec{\agent}\varphi \then \nec{\agent}\pos{\agent}\varphi$ & \axiomname{5$^{-1}$} \\ \hline %++++++++++++++++++--
$(1,0,0,0)$ & $\pos{\agent}\varphi \then \varphi$ &  \axiomname{Ban}\\ \hline %ok%ok
$(1,0,0,1)$ & $\pos{\agent}\varphi \then \pos{\agent}\varphi$ &  classical \\ \hline  %--
$(1,0,1,0)$ & $\pos{\agent}\varphi \then \nec{\agent}\varphi$ & \axiomname{F} \\ \hline % okok
$(1,0,1,1)$ & $\pos{\agent}\varphi \then \nec{\agent}\pos{\agent}\varphi$ & \axiomname{5} \\ \hline % okok
$(1,1,0,0)$ & $\pos{\agent}\nec{\agent}\varphi \then \varphi$ &  \axiomname{B}\\ \hline %ok%ok
$(1,1,0,1)$ & $\pos{\agent}\nec{\agent}\varphi \then \pos{\agent}\varphi$ & \axiomname{5$^{-1}$} \\ \hline % ++++++++++++++++++
$(1,1,1,0)$ & $\pos{\agent}\nec{\agent}\varphi \then \nec{\agent}\varphi$ & \axiomname{5} \\ \hline % okok
$(1,1,1,1)$ & $\pos{\agent}\nec{\agent}\varphi \then \nec{\agent}\pos{\agent}\varphi$ & \axiomname{G1}, converse of \axiomname{McK} \\ \hline %ok
\end{tabular}
\caption{Axioms $\G{\gp,\gq,\gr,\gs}{\agent}$, with $\gp,\gq,\gr,\gs \in \Set{0,1}$.}
\label{table:axioms}
\end{table}


==> tables/table-rules.tex <==
{\tiny
\begin{sidewaystable}
\begin{tabular}{|c|c|c|c|p{5.5cm}|c|}\hline
(p,q,r,s)   &       Name      & Axiom & Condition & First-Order & Resolution \\ \hline
$(0,0,1,1)$ & \axiomname{B}   & $\varphi \then \nec{\agent}\pos{\agent}\varphi$ & symmetric & $\forall w, w' (w \relation{R}{\agent} w' \then w' \relation{R}{\agent} w)$ & {\footnotesize\textcolor{red}{
$
\begin{array}{lrcl}
\mbox{[SYM]} & \universal(l_1 & \then & \nec{\agent} l) \\ \cline{2-4}
& \universal(\constant{true} & \then & \neg \newpos{\agent,l_1} \lor l)
\end{array}
$
}}\\
$(1,1,0,0)$ &                 & $\pos{\agent}\nec{\agent}\varphi \then \varphi$ & & & \\ \hline
$(0,0,1,0)$ & \axiomname{Ban} & $\varphi \then \nec{\agent}\varphi$ &  &$\forall w, w' (w \relation{R}{\agent} w' \then w = w')$ &{\footnotesize\textcolor{red}{
$
\begin{array}{lrcl}
\mbox{[BAN]} & \universal(l_1 & \then & \neg\nec{\agent}\neg l) \\ \cline{2-4}
& \universal(\constant{true} & \then & \neg l_1 \lor  l)
\end{array}
$
}} \\
$(1,0,0,0)$ &                 & $\pos{\agent}\varphi \then \varphi$ &  & &\\ \hline
$(0,1,0,1)$ & \axiomname{D}   & $\nec{\agent}\varphi \then \pos{\agent}\varphi$ & serial & $\forall w \exists w' (w \relation{R}{\agent} w')$ & {\footnotesize
$
\begin{array}{lrcl}
\mbox{[SER ]} & \universal(l_1 & \then & \nec{\agent}l) \\ \cline{2-4}
              & \universal(l_1 & \then & \neg \nec{\agent}\neg l) \\     
\end{array}
$
}\\\hline
$(1,0,1,0)$ & \axiomname{F}   & $\pos{\agent}\varphi \then \nec{\agent}\varphi$ & functional & $\forall w, w', w'' (w \relation{R}{\agent} w' \land w \relation{R}{\agent} w'') \then w' = w''$ &{\footnotesize\textcolor{red}{
$
\begin{array}{lrcl}
\mbox{[FUN]} & \universal(l_1 & \then & \neg\nec{\agent}\neg l) \\ \cline{2-4}
& \universal(l_1 & \then & \nec{\agent}l)
\end{array}
$
}}  \\ \hline
$(0,0,0,1)$ & \axiomname{T}   & $\varphi \then \pos{\agent}\varphi$ & reflexive & $\forall w  (w \relation{R}{\agent} w)$ & {\footnotesize
$
\begin{array}{lrcl}
\mbox{[REF]} & \universal(l_1 & \then & \nec{\agent}l) \\  \cline{2-4}
& \universal(\constant{true} & \then & \neg l_1 \vee l)
\end{array}
$
}\\
$(0,1,0,0)$ &                 & $\nec{\agent}\varphi \then \varphi$ &           & & \\ \hline
$(1,0,1,1)$ & \axiomname{5}   & $\pos{\agent}\varphi \then \nec{\agent}\pos{\agent}\varphi$ & euclidian & $\forall w, w', w'' ((w \relation{R}{\agent} w' \land w \relation{R}{\agent} w'') \then w' \relation{R}{\agent} w'')$ &{\footnotesize\textcolor{red}{ 
$
 \begin{array}{lrcl}
 \mbox{[EUC1]} & \universal(l_1 & \then & \neg \nec{\agent}\neg l) \\ \cline{2-4}
 & \universal(\newpos{\agent,l_1} & \then & \nec{\agent} \newpos{\agent,l})\\
\\
\\
 \end{array}$
}}\\
$(1,1,1,0)$ &                 & $\pos{\agent}\nec{\agent}\varphi \then \nec{\agent}\varphi$ & & & {\footnotesize\textcolor{red}{
$\begin{array}{lrcl}
\mbox{[EUC2]} &\universal( l_1  & \then &  \nec{\agent} l)\\ \cline{2-4}
              & \universal(\newpos{\agent,l_1} & \then & \nec{\agent} \newpos{\agent,l})\\
\end{array}
$
}}\\ \hline
$(1,1,1,1)$ & \axiomname{G1}, \axiomname{C}  & $\pos{\agent}\nec{\agent}\varphi \then \nec{\agent}\pos{\agent}\varphi$ & diamond, convergent & $\forall w, w', w'' (w \relation{R}{\agent} w' \land w \relation{R}{\agent} w'') \then \exists w''' (w' \relation{R}{\agent} w''' \land w'' \relation{R}{\agent} w''')$ & {\footnotesize\textcolor{red}{
$
\begin{array}{lrcl}
\mbox{[\rulename{InRES1}]} 
              &\universal( l & \then & \nec{\agent} l') \\ \cline{2-4}
              &\universal( \newpos{\agent,l} & \then & \nec{\agent} \newpos{\agent,l'}) \\
          \end{array}
$
}}
\\ \hline
$(0,1,1,1)$ & \axiomname{5$^{-1}$} & $\nec{\agent}\varphi \then \nec{\agent}\pos{\agent}\varphi$ & {\textcolor{red}{??? name for this}} & 
\textcolor{blue}{$\forall w, w' (w \relation{R}{\agent} w' \then \exists w''(w \relation{R}{\agent} w'' \land w' \relation{R}{\agent} w'')$}
%$\forall w, w' (w \relation{R}{\agent} w' \then w' \relation{R}{\agent} w')$ 
& {\footnotesize\textcolor{red}{
$
\begin{array}{lrcl}
\mbox{[???]} & \universal(l_1 & \then & \nec{\agent} l) \\ \cline{2-4}
             & \universal(\newpos{\agent,l_1} & \then & \neg\nec{\agent}\neg l) \\ 
\end{array}
$
}}\\ 

$(1,1,0,1)$ &  & $\pos{\agent}\nec{\agent}\varphi \then \pos{\agent}\varphi$ & & Ex 3.4.1 pg.74 & \\ \hline
\end{tabular}
\label{table:rules}
\caption{Resolution Rules}
\end{sidewaystable}
}

